Code Rate Optimization via Neural Polar Decoders

This paper proposes a method to optimize communication code rates via the application of neural polar decoders (NPDs). Employing this approach enables simultaneous optimization of code rates over input distributions while providing a practical coding scheme within the framework of polar codes. The proposed approach is designed for scenarios where the channel model is unknown, treating the channel as a black box that produces output samples from input samples. We employ polar codes to achieve our objectives, using NPDs to estimate mutual information (MI) between the channel inputs and outputs, and optimize a parametric model of the input distribution. The methodology involves a two-phase process: a training phase and an inference phase. In the training phase, two steps are repeated interchangeably. First, the estimation step estimates the MI of the channel inputs and outputs via NPDs. Second, the improvement step optimizes the input distribution parameters to maximize the MI estimate obtained by the NPDs. In the inference phase, the optimized model is used to construct polar codes. This involves incorporating the Honda-Yamamoto (HY) scheme to accommodate the optimized input distributions and list decoding to enhance decoding performance. Experimental results on memoryless and finite-state channels (FSCs) demonstrate the effectiveness of our approach, particularly in cases where the channel's capacity-achieving input distribution is non-uniform. For these cases, we show significant improvements in MI and bit error rates (BERs) over those achieved by uniform and independent and identically distributed (i.i.d.) input distributions, validating our method for block lengths up to 1024. This scalable approach has potential applications in real-world communication systems, bridging theoretical capacity estimation and practical coding performance.

==> figures/optimized_ber_trapdoor.tex <==
\begin{tikzpicture}
\definecolor{darkblue}{rgb}{0,0,0.55}
\definecolor{darkgreen}{rgb}{0,0.39,0}
\definecolor{maroon}{rgb}{0.5,0,0}
\definecolor{plum}{rgb}{0.56,0.27,0.52}
\definecolor{darkorange}{rgb}{0.8,0.33,0} 
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}



% First plot
\begin{axis}[
    name=plot1,
    title={Optimized Input Distribution},
    xlabel={\textcolor{dimgray85}{$\displaystyle \log_2(N)$}},
    ylabel={\textcolor{dimgray85}{BER}},
    ymode=log,
    ymin=5e-4, ymax=0.3,
        xmajorgrids,
    ymajorgrids,
    % colorbar,
    colormap/viridis,
    % colorbar style={
    %   title={$L$},
    %   ytick={0, 2, 4, 6, 8},
    %   yticklabels={$1$, $4$, $16$, $64$, $256$},
    % },
  ]
    \addplot [scatter,
      only marks,
      scatter src=explicit,
    ]
    table[meta expr=log10(\thisrow{meta})/log10(2)]{
n	ber	meta
3	0.064747628	1
3	0.041942474	2
3	0.042535748	4
3	0.041245877	8
3	0.042362432	16
3	0.042615739637500656	32
3	0.042112278	64
3	0.042082293	128
3	0.04217558	256
4	0.021414293	1
4	0.013846410460945133	2
4	0.013383308660233396	4
4	0.013588206216670584	8
4	0.013579877055716002	16
4	0.013449942	32
4	0.013581542882813267	64
4	0.013270031967829133	128
4	0.013226720294256556	256
5	0.049235383	1
5	0.027340497	2
5	0.02234716	4
5	0.021525071205823556	8
5	0.021849076	16
5	0.021642513	32
5	0.0222014	64
5	0.021878227978974565	128
5	0.0222672	256
6	0.10829665127045092	1
6	0.041750325	2
6	0.019243178	4
6	0.012464967293032762	8
6	0.011623788	16
6	0.011307546009664712	32
6	0.011414293	64
6	0.011471464044001626	128
6	0.011544627	256
7	0.1430363286897421	1
7	0.050265261	2
7	0.020511118	4
7	0.011018216690771852	8
7	0.008298596	16
7	0.007327317	32
7	0.007004145	64
7	0.007121733	128
7	0.006922225	256
8	0.17299448637340192	1
8	0.066197295	2
8	0.029499172597931795	4
8	0.014505394677036274	8
8	0.008365327	16
8	0.00561729	32
8	0.004496673	64
8	0.004089916	128
8	0.00392539	256
9	0.18519358013518275	1
9	0.074962519	2
9	0.029566688	4
9	0.013192080582898372	8
9	0.007291648	16
9	0.004785793	32
9	0.003923676	64
9	0.003442788	128
9	0.003352099	256
10	0.21778973597697385	1
10	0.089710621	2
10	0.036836154	4
10	0.016564309561787092	8
10	0.008230579	16
10	0.0045782	32
10	0.002955124	64
10	0.002060192	128
10	0.001633584	256
};
    % Adding lines between points with the same meta value
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.064747628) (4,0.021414293) (5,0.049235383) (6,0.10829665127045092) (7,0.1430363286897421) (8,0.17299448637340192) (9,0.18519358013518275) (10,0.21778973597697385)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.041942474) (4,0.013846410460945133) (5,0.027340497) (6,0.041750325) (7,0.050265261) (8,0.066197295) (9,0.074962519) (10,0.089710621)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.042535748) (4,0.013383308660233396) (5,0.02234716) (6,0.019243178) (7,0.020511118) (8,0.029499172597931795) (9,0.029566688) (10,0.036836154)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.041245877) (4,0.013588206216670584) (5,0.021525071205823556) (6,0.012464967293032762) (7,0.011018216690771852) (8,0.014505394677036274) (9,0.013192080582898372) (10,0.016564309561787092)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.042362432) (4,0.013579877055716002) (5,0.021849076) (6,0.011623788) (7,0.008298596) (8,0.008365327) (9,0.007291648) (10,0.008230579)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.042615739637500656) (4,0.013449942) (5,0.021642513) (6,0.011307546009664712) (7,0.007327317) (8,0.00561729) (9,0.004785793) (10,0.0045782)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.042112278) (4,0.013581542882813267) (5,0.0222014) (6,0.011414293) (7,0.007004145) (8,0.004496673) (9,0.003923676) (10,0.002955124)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.042082293) (4,0.013270031967829133) (5,0.021878227978974565) (6,0.011471464044001626) (7,0.007121733) (8,0.004089916) (9,0.003442788) (10,0.002060192)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.04217558) (4,0.013226720294256556) (5,0.0222672) (6,0.011544627) (7,0.006922225) (8,0.00392539) (9,0.003352099) (10,0.001633584)};

\end{axis}

% Second plot
\begin{axis}[
    name=plot2,
    at={(plot1.east)},
    anchor=west,
    xshift=2.5cm, % Adjust space between the plots
    title={Uniform i.i.d. Input distribution},
    xlabel={\textcolor{dimgray85}{$\displaystyle \log_2(N)$}},
    xmajorgrids,
    ymajorgrids,
    ymode=log,
    ymin=5e-4, ymax=0.3,
    colorbar,
    colormap/viridis,
    colorbar style={
      title={$L$},
      ytick={0, 2, 4, 6, 8},
      yticklabels={$1$, $4$, $16$, $64$, $256$},
    },
  ]
    \addplot [scatter,
      only marks,
      scatter src=explicit,
    ]
    table[meta expr=log10(\thisrow{meta})/log10(2)]{
n	ber	meta
3	0.088624473	1
3	0.087686159	2
3	0.085893722	4
3	0.086226888	8
3	0.087552892	16
3	0.086396803	32
3	0.088019325	64
3	0.087034632	128
3	0.087297939	256
4	0.093678967	1
4	0.067218059	2
4	0.067641181	4
4	0.068572382	8
4	0.067432951	16
4	0.067866068	32
4	0.068087624	64
4	0.06744659	128
4	0.067809887	256
5	0.08303753	1
5	0.062622855	2
5	0.060338164421169835	4
5	0.061031984	8
5	0.061872397	16
5	0.060587207	32
5	0.060814593	64
5	0.060987235	128
5	0.060616438538089366	256
6	0.10522707646405167	1
6	0.079339529	2
6	0.075986806	4
6	0.076211094	8
6	0.075901648	16
6	0.075887256	32
6	0.076285856	64
6	0.075144085	128
6	0.077165883	256
7	0.1419422801637458	1
7	0.096227047	2
7	0.085188346	4
7	0.08090054	8
7	0.080372357	16
7	0.081678109	32
7	0.081542436	64
7	0.080916224	128
7	0.08102739	256
8	0.1538845170352229	1
8	0.091964825	2
8	0.070747535	4
8	0.063440324	8
8	0.061241132320200904	16
8	0.060719223738689994	32
8	0.06119996	64
8	0.060597373	128
8	0.060907048	256
9	0.18572079291781016	1
9	0.091246122	2
9	0.053168704	4
9	0.038915374	8
9	0.033923912	16
9	0.032369606861373086	32
9	0.03119247	64
9	0.030746485	128
9	0.030401421304353183	256
10	0.1986497927940705	1
10	0.093933052	2
10	0.051945539	4
10	0.034541069	8
10	0.027927402990613904	16
10	0.024880079	32
10	0.023378322	64
10	0.022803098803893425	128
10	0.022485746682911895	256
};

% Adding lines between points with the same meta value
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.088624473) (4,0.093678967) (5,0.08303753) (6,0.10522707646405167) (7,0.1419422801637458) (8,0.1538845170352229) (9,0.18572079291781016) (10,0.1986497927940705)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.087686159) (4,0.067218059) (5,0.062622855) (6,0.079339529) (7,0.096227047) (8,0.091964825) (9,0.091246122) (10,0.093933052)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.085893722) (4,0.067641181) (5,0.060338164421169835) (6,0.075986806) (7,0.085188346) (8,0.070747535) (9,0.053168704) (10,0.051945539)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.086226888) (4,0.068572382) (5,0.061031984) (6,0.076211094) (7,0.08090054) (8,0.063440324) (9,0.038915374) (10,0.034541069)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.087552892) (4,0.067432951) (5,0.061872397) (6,0.075901648) (7,0.080372357) (8,0.061241132320200904) (9,0.033923912) (10,0.027927402990613904)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.086396803) (4,0.067866068) (5,0.060587207) (6,0.075887256) (7,0.081678109) (8,0.060719223738689994) (9,0.032369606861373086) (10,0.024880079)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.088019325) (4,0.068087624) (5,0.060814593) (6,0.076285856) (7,0.081542436) (8,0.06119996) (9,0.03119247) (10,0.023378322)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.087034632) (4,0.06744659) (5,0.060987235) (6,0.075144085) (7,0.080916224) (8,0.060597373) (9,0.030746485) (10,0.022803098803893425)};
    \addplot[dimgray85, line width=0.1pt] coordinates {(3,0.087297939) (4,0.067809887) (5,0.060616438538089366) (6,0.077165883) (7,0.08102739) (8,0.060907048) (9,0.030401421304353183) (10,0.022485746682911895)};
\end{axis}


\end{tikzpicture}
